Large-scale Kernel Methods and Applications to Lifelong Robot Learning

As the size and richness of available datasets grow larger, the opportunities for solving increasingly challenging problems with algorithms learning directly from data grow at the same pace. Consequently, the capability of learning algorithms to work with large amounts of data has become a crucial scientific and technological challenge for their practical applicability. Hence, it is no surprise that large-scale learning is currently drawing plenty of research effort in the machine learning research community. In this thesis, we focus on kernel methods, a theoretically sound and effective class of learning algorithms yielding nonparametric estimators. Kernel methods, in their classical formulations, are accurate and efficient on datasets of limited size, but do not scale up in a cost-effective manner. Recent research has shown that approximate learning algorithms, for instance random subsampling methods like Nystr\"om and random features, with time-memory-accuracy trade-off mechanisms are more scalable alternatives. In this thesis, we provide analyses of the generalization properties and computational requirements of several types of such approximation schemes. In particular, we expose the tight relationship between statistics and computations, with the goal of tailoring the accuracy of the learning process to the available computational resources. Our results are supported by experimental evidence on large-scale datasets and numerical simulations. We also study how large-scale learning can be applied to enable accurate, efficient, and reactive lifelong learning for robotics. In particular, we propose algorithms allowing robots to learn continuously from experience and adapt to changes in their operational environment. The proposed methods are validated on the iCub humanoid robot in addition to other benchmarks.

==> chapters/appRFerrDec.tex <==

In the next theorem, by using analytic arguments, we decompose the excess risk in three terms.
\bt[Analytic Decomposition]\label{thm:geo-dec}
Under Assumptions~\ref{ass:noise},~\ref{ass:psi-continuous-bounded},~\ref{ass:kerrf-sep}, and Eq.~\ref{eq:source} of Assumption~\ref{ass:source-condition}, let $\tilde{f}_{m,\la}$ as in Eq.~\eqref{eq:RF-KRLS}. For any $\la > 0$ and $m > 0$, the following holds
\eqal{
|\EE(\tilde{f}_{m,\la}) - \EE(\frho)|^{1/2}  \;\;\leq\;\; \beta\;(\;\;\underbrace{{\cal S}(\la, m, n)}_\textrm{Sample Error}\;\; + \underbrace{{\cal C}(\la,m)}_\textrm{Computational Error} + \underbrace{R\la^{v}}_\textrm{Approximation Error})
}
where $v = \min(r,1)$ and
\begin{enumerate}
\item $\beta = (1 - \beta_1)^{-1}(1-\beta_2)^{-1/2}$, with $\beta_1 = \la_{\max}(\tCl^{-1/2}(\tC - \tCn)\tCl^{-1/2})$ and $\beta_2 = \la_{\max}(\Ll^{-1/2}(L - \tL)\Ll^{-1/2})$;
\item ${\cal C}(\la, m) = R\la^{1/2}\nor{\Ll^{-1/2}(L - \tL)}^{2v-1}\nor{\Ll^{-1/2}(L - \tL)\Ll^{-1/2}}^{2-2v}$ and
\item ${\cal S}(\la,m,n) = \nor{\tCl^{-1/2}\tSn^*(y - S_n\fh)} + \nor{\fh}_\hh \left( \nor{\tCl^{-1/2}(\tSn^*S_n - \tS^*S)} + \nor{\tCl^{-1/2}(\tC - \tCn)}\right)$.
\end{enumerate}
\et
The proof is based on the combinations of Lemma~\ref{lm:bounding-A},~\ref{lm:bounding-B} and is given at the end of this section.
\blm\label{lm:bounding-A} Under the same assumptions of Thm.~\ref{thm:geo-dec} we have that
\eqals{
\nor{\tilde{f}_{m,\la} - \tL \tLl^{-1}\frho}_\rhox \leq \beta\,{\cal S}(\la,m,n),
}
with $\beta$ and ${\cal S}(\la,m,n)$ defined as in points 1 and 3 of Thm.~\ref{thm:geo-dec}.
\elm
\bpr First of all note that according to Eq.~\ref{eq:RF-KRLS} and the definition of $\tS$ in Def.~\ref{def:all-ops},~\ref{def:all-ops-tilde}, we have $\tilde{f}_{m,\la} = \tS\tCnl^{-1}\tSn^*\yn$. Moreover, since $\tL = \tS \tS^*$, then $\tL \tLl^{-1} = \tS\tCl^{-1}\tS^*$ (see Def.~\ref{def:all-ops},~\ref{def:all-ops-tilde} and Rem.~\ref{rem:S-C-L}). Thus we have
$$\nor{\tilde{f}_{m,\la} - \tL \tLl^{-1}\frho}_\rhox = \nor{\tS\tCnl^{-1}\tSn^*\yn - \tS\tCl^{-1}\tS^*\frho}_\rhox.$$
By Prop.~\ref{prop:fh}, we have that there exists $\fh \in \hh$ such that $\frho = S\fh$. Thus, by adding and subtracting $\tS\tCnl^{-1}\tS^* \S \fh$, we have
\eqals{
 \nor{\tS\tCnl^{-1}\tSn^*\yn - \tS\tCl^{-1}\tS^*\frho}_\rhox & \leq \underbrace{\nor{\tS\tCnl^{-1}(\tSn^*\yn - \tS^*\S \fh)}_\rhox}_{A.1} +  \underbrace{\nor{\tS(\tCnl^{-1} - \tCl^{-1})\tS^*S\fh}_\rhox}_{A.2}.
}
By multiplying and dividing by $\tCl^{1/2}$ we split the term in
\eqals{
A.1 & \leq \nor{\tS\tCnl^{-1}\tCl^{1/2}}\nor{\tCl^{-1/2}(\tSn^*y - \tS^*\S \fh)} \\
& = \nor{\tS\tCnl^{-1}\tCl^{1/2}}\nor{\tCl^{-1/2}((\tSn^*y - \tSn^*\Sn \fh) + (\tSn^*\Sn \fh - \tS^*\S \fh))} \\
& \leq \nor{\tS\tCnl^{-1}\tCl^{1/2}}\left(\nor{\tCl^{-1/2}\tSn^*(y - \Sn \fh)} + \nor{\tCl^{-1/2}(\tSn^*\Sn -  \tS^*\S)\fh}\right)\\
& \leq \nor{\tS\tCnl^{-1}\tCl^{1/2}}\left(\nor{\tCl^{-1/2}\tSn^*(y - \Sn \fh)} + \nor{\fh}_\hh\nor{\tCl^{-1/2}(\tSn^*\Sn -  \tS^*\S)}\right)
}
For the term A.2, we have
\eqals{
A.2 &= \nor{\tS\tCnl^{-1}(\tC - \tCn)\tCl^{-1}\tS^*S\fh}_\rhox \\
& \leq \nor{\tS\tCnl^{-1}\tCl^{1/2}}\nor{\tCl^{-1/2}(\tC - \tCn)}\nor{\tCl^{-1}\tS^*S}\nor{\fh}_\hh
}
Noting that $\tS\tCl^{-2}\tS^* = \tLl^{-1}\tL\tLl^{-1}$ and $\nor{\tL^{1/2}\tLl^{-1/2}} \leq 1$, we have
\eqals{
\nor{\tCl^{-1}\tS^*S} & = \nor{S^*\tS\tCl^{-2}\tS^*S}^{1/2} = \nor{S^*\tL^{-1}\tL\tLl^{-1}S}^{1/2} = \nor{\tL^{1/2}\tLl^{-1}S} \\
& \leq \nor{\tL^{1/2}\tLl^{-1/2}}\nor{\tLl^{-1/2}S} \leq \nor{\tLl^{-1/2}S}.
} 
Moreover
\eqals{
\nor{\tLl^{-1/2}S} &= \nor{\tLl^{-1/2}L\tLl^{-1/2}}^{1/2} = \nor{\tLl^{-1/2}L^{1/2}} \leq (1 - \beta_2)^{-1/2},
}
where the last step is due to Prop~\ref{prop:invAtoinvB}. Finally,
$$ A.2 \leq (1 - \beta_2)^{-1/2}\nor{\tS\tCnl^{-1}\tCl^{1/2}}\nor{\tCl^{-1/2}(\tC - \tCn)}\nor{\fh}_\hh.$$
Therefore, we have
\eqals{ \nor{\tilde{f}_{m,\la} - \tL \tLl^{-1}\frho}_\rhox \leq A.1 + A.2 \leq (1 - \beta_2)^{-1/2}\nor{\tS\tCnl^{-1}\tCl^{1/2}}\,{\cal S}(\la,m,n).
}
Finally note that 
$\nor{\tS\tCl^{-1/2}}^2 = \nor{\tCl^{-1/2}\tC\tCl^{-1/2}} \leq 1,$ thus we have that
$$\nor{\tS\tCnl^{-1}\tCl^{1/2}} \leq  \nor{\tS\tCl^{-1/2}} \nor{\tCl^{1/2}\tCnl^{-1}\tCl^{1/2}} = \nor{\tCnl^{-1/2}\tCl^{1/2}}^2,$$
and so $\nor{\tS\tCnl^{-1}\tCl^{1/2}} \leq \nor{\tCnl^{-1/2}\tCl^{1/2}}^2 \leq (1 - \beta_1)^{-1}$ by Proposition~\ref{prop:invAtoinvB}.
\epr
%
%
\blm\label{lm:bounding-B}
Under the same assumptions of Thm.~\ref{thm:geo-dec} we have
\eqals{
	\nor{\frho - \tL \tLl^{-1}\frho}_\rhox \leq R(1-\beta_2)^{-1/2}~\left(\la^{v} + \la^{1/2}\nor{\Ll^{-1/2}(L - \tL)}^{2v-1}\nor{\Ll^{-1/2}(L - \tL)\Ll^{-1/2}}^{2-2v}\right).
}
with $\beta_2$ in point 1 of Thm.~\ref{thm:geo-dec} and $v = \min(r,1)$.
\elm
\bpr
By Assumption~\ref{ass:source-condition}, we have that
\eqals{\nor{\frho - \tL \tLl^{-1}\frho}_\rhox &= \nor{(I - \tL \tLl^{-1})\frho}_\rhox = \la\nor{\tLl^{-1}\frho}_\rhox = \la\nor{\tLl^{-1}\L^v\L^{-v}\frho}_\rhox\\
& \leq \la\nor{\tLl^{-1}\L^v}\nor{\L^{-v}\frho}_\rhox \leq R\la\nor{\tLl^{-1}\L^v}
}
where the last step is due to $\nor{\L^{-v}\frho}_\rhox \leq \nor{\L^{-r}\frho}_\rhox \leq R$.
%by the spectral theorem (see \cite{reed1980methods} Thm.~VII.2).
Now note that 
$$\tLl^{-1} = \Ll^{-1} + (\tLl^{-1} - \Ll^{-1}) = \Ll^{-1} + \tLl^{-1}(L - \tL)\Ll^{-1} =  (I + \tLl^{-1}(L - \tL))\Ll^{-1},$$
therefore, by denoting $u = 2 - 2v$ (note that since $v \in [1/2,1]$, then $u \in [0,1]$), we have
\eqals{
\nor{\tLl^{-1} L^v} &\leq \nor{(I + \tLl^{-1}(L - \tL))\Ll^{-1} L^v} \\
& \leq \nor{(I + \tLl^{-1}(L - \tL))\Ll^{-u/2}}\nor{\Ll^{-v} L^v} \\
& \leq \nor{\Ll^{-u/2}} + \nor{\tLl^{-1}(L - \tL)\Ll^{-u/2}}\\
& \leq \la^{-u/2} + \nor{\tLl^{-1/2}}\nor{\tLl^{-1/2}\Ll^{1/2}}\nor{\Ll^{-1/2}(L - \tL)\Ll^{-u/2}} \\
& \leq \la^{-u/2} + \la^{-1/2}(1-\beta_2)^{-1/2}\nor{\Ll^{-1/2}(L - \tL)\Ll^{-u/2}},
}
where $\nor{\tLl^{-1/2}\Ll^{1/2}} \leq (1-\beta_2)^{-1/2}$, by Proposition~\ref{prop:invAtoinvB}.
Then we have
\eqals{
\nor{\frho - \tL \tLl^{-1}\frho}_\rhox &\leq \la \nor{\tLl^{-1}S \fh}_\rhox  \leq R\la^{1-u/2} +  R\la^{1/2}(1-\beta_2)^{-1/2}\nor{\Ll^{-1/2}(L - \tL)\Ll^{-u/2}}\\
& \leq (1-\beta_2)^{-1/2}\left(R\la^{v} + R\la^{1/2}\nor{\Ll^{-1/2}(L - \tL)\Ll^{-u/2}}\right).
}
The last step consists in applying Proposition~\ref{prop:interp} on $\nor{\Ll^{-1/2}(L - \tL)\Ll^{-u/2}}$ by setting $X = \Ll^{-1/2}(L - \tL)$, $A = \Ll^{-1/2}$ and $\sigma = u$, the result is
$$\nor{\Ll^{-1/2}(L - \tL)\Ll^{-u/2}} \leq \nor{\Ll^{-1/2}(L - \tL)}^{2v-1}\nor{\Ll^{-1/2}(L - \tL)\Ll^{-1/2}}^{2-2v}.$$
\epr
%
%
\bpr[Proof of Theorem~\ref{thm:geo-dec}]
Note that, under Assumption~\ref{ass:noise}, we have
$$\EE(\tilde{f}_{m,\la}) - \EE(\frho) = \int_X (\tilde{f}_{m,\la}(x) - \frho(x))^2 d\rhox(x) = \nor{\tilde{f}_{m,\la} - \frho}^2_\rhox.$$
To bound the excess risk, we introduce the function $\tL \tLl^{-1} \frho$ that is a regularized projection of $\frho$ on the range of $\tL$. We have
\be\label{eq:geo-dec-AB}
|\EE(\tilde{f}_{m,\la}) - \EE(\frho)|^{1/2} \leq nor{\tilde{f}_{m,\la} - \tL \tLl^{-1}\frho}_\rhox + \nor{\tL \tLl^{-1}\frho - \frho}_\rhox.
\ee
%
By applying Lemma~\ref{lm:bounding-A}, Lemma~\ref{lm:bounding-B}, we have
\eqals{
|\EE(\tilde{f}_{m,\la}) - \EE(\frho)|^{1/2} \leq A + B \leq \beta\left({\cal S}(\la, m, n) \;\;+\;\; {\cal C}(\la, m) \;\;+\;\;  R\la^{v}\right).
}
\epr

==> chapters/falcon.tex <==
--- No (?) ---

==> chapters/spectral-filters.tex <==
In this Section, we review the concept of \textit{spectral regularization}, a general formalism describing a large class of regularization methods giving rise to consistent learning algorithms.

\section{Introduction}
Spectral regularization originates from the inverse problems literature, drawing in particular from methods to invert matrices in a numerically stable way.
The keystone concept of spectral regularization is that the same principles allowing for numerically stable inversion can be shown to prevent overfitting in a SLT framework.
Different spectral methods have a common derivation, but result in different regularized learning algorithms in terms of computational complexity and theoretical properties.
As we have seen in Chapter \ref{Chap:SLT}, a learning problem can be framed as the minimization of the expected risk on a suitable hypotheses space.
In practical algorithms, the empirical risk is introduced as a proxy of the expected risk, and a regularizer is used to penalize too complex solutions which could be unstable with respect to sampling and noise.
In the case of the square loss, we have also seen (Chapters \ref{Chap:SLT}, \ref{Chap:kernelMethods}) that finding a generalizing solution to a learning problem depends on the inversion of a linear operator (matrix), be it the correlation matrix $X^\top X$ for RLS or the kernel matrix $K_n$ for KRLS.
The spectral regularization literature includes a rich variety of methods allowing to invert linear operators in a stable way.
In fact, finding a solution to an ill-posed problem may involve the inversion of a linear operator with high condition number\footnote{The condition number of a matrix $A$ is defined as $\kappa(A) = \sigma_{\text{max}} / \sigma_{\text{min}}$, where $\sigma_{\text{max}}, \sigma_{\text{min}}$ are the maximal and minimal singular values of $A$ respectively.}, or, similarly, with unbounded inverse.
In this case, small eigenvalues are strongly susceptible to sampling and noise, therefore resulting in numerically unstable matrix inversion and overfitting.
In other words, small noise-dependent perturbations of the eigenvalues yield large changes of the inverse.
In general, spectral regularization methods act on the eigenvalues of the matrix to stabilize the inversion.
This is done by replacing the original unbounded operator with a \textit{regularization operator} \cite{engl...} which allows to control the condition number via a regularization parameter.
In the following, we will review the main spectral regularization methods of interest for the scope of this work.

\section{Tikhonov}
Given a finite training set sampled from some fixed unknown distribution and a loss function, we have seen that the Tikhonov regularization\index{Tikhonov regularization} can be used as a general approach to approximatively solve the learning problem. More precisely, given a training set and a loss function, we have considered learning methods induced by minimization problems of the form
\begin{equation}\label{TikReg}
\min_{f\in \hh} \En(f)+\la R(f), \quad \la >0.
\end{equation}
The idea is that for a suitable   hypothesis space $\hh$, and a  regularizer $R:\hh\to [0,\infty)$, the solution of the above problem should provide an approximate solution of the expected risk minimization problem
$$
\inf_{f\in \F} \EE(f).
$$
We have discussed in detail the case where $\hh$ is a RKHS\index{reproducing kernel Hilbert space} and $R$ the corresponding squared norm, and we will later see several other instances of the above idea.
Indeed, approaches based on penalization of the empirical risk are so common that the term regularization is often identified with schemes of the form~\eqref{TikReg}.
Next, we discuss other principles leading to sound regularized learning methods, when considering hypothesis spaces which are RKHS.

\section{Truncated SVD}
		
$$
\hat{X}^\top \hat{X} = V\Sigma V^\top, \quad\quad w_M = (\hat{X}^\top \hat{X})^{-1}_M \hat{X}^\top \hat{y}
$$

\begin{itemize}
\item $(\hat{X}^\top \hat{X})^{-1}_M = V \Sigma_M^{-1} V^\top$
%\item $\Sigma_M^{-1} = \textrm{diag}(\sigma_1^{-1},\dots,\sigma_{\color{red}M}^{-1}, 0\dots, 0)$ 
\item $\Sigma_M^{-1} = \textrm{diag}(\sigma_1^{-1},\dots,\sigma_{M}^{-1}, 0\dots, 0)$ 
\end{itemize}

Also known as principal component regression (PCR)


%\begin{frame}{Principal component analysis (PCA)}
%Dimensionality reduction
%$$\hat{X}^\top \hat{X} = V\Sigma V^\top$$
%\vfill
%\begin{columns}[T]
%\begin{column}[T]{4cm} 
%Eigenfunctions are directions, of
%\bi
%\item maximum variance
%\item best reconstruction
%\ei
%\end{column}
%\begin{column}[T]{4cm} 
%\begin{center}
%\includegraphics[width=5cm]{figures/points.png}
%\end{center}
%\end{column}
%\end{columns}
%
%\end{frame}

%\begin{frame}{TSVD and PCA}
$$
TSVD \quad \Leftrightarrow \quad PCA + ERM
$$
Regularization by projection.\\

Note:  PCA + ERM can be used as regularization for other loss functions


\subsection{TSVD with feature maps}
Non-linear function
$$f(x) = \sum_{i=1}^p w_i \phi_i(x) = \Phi(x) ^\top w$$
with
$$ w = (\widehat{\Phi}^\top\widehat{\Phi})^{-1}_M \widehat{\Phi}^\top\hat{y}$$
Let $\widehat{\Phi} = (\Phi(x_1),\dots \Phi(x_n))^\top \in \R^{n \times p}.$
$$\widehat{\Phi}^\top\widehat{\Phi} = V \Sigma V^\top, \quad (\widehat{\Phi}^\top\widehat{\Phi})^{-1}_M = V \Sigma^{-1}_M V^\top$$

$$\Sigma = \textrm{diag}(\sigma_1,\dots,\sigma_p), \quad \Sigma^{-1}_M = \textrm{diag}(\sigma_1^{-1},\dots,\sigma_M^{-1},0,\dots)$$

\subsection{TSVD/PCR with kernels}
$$f(x) = \sum_{i=1}^n K(x, x_i) c_i, \quad c = (\widehat{K})_{M}^{-1} \hat{y}$$

$$ \widehat{K}_{ij} = K(x_i, x_j), \quad \widehat{K} = U \Sigma U^\top, \quad \Sigma = (\sigma_1,\dots,\sigma_n),$$
$$ \widehat{K}_M^{-1} = U \Sigma^{-1}_M U^\top, \quad \Sigma^{-1}_M = (\sigma_1^{-1},\dots,\sigma_M^{-1},0,\dots),$$
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Iterative Regularization via Early Stopping}\index{iterative regularization}\index{early stopping}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The idea of iterative regularization is to  recursively define a sequence of empirical solutions: the first few iterations provide simple solutions, whereas running the iteration for too long
could lead to  overfitting. Therefore early termination of the iteration can be interpreted as having a regularizing effect. We begin discussing this idea first for least squares\index{least squares} loss and then for general convex loss functions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Early Stopping for Least Squares}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We begin considering the linear kernel and let $\Xn,\Yn$ be the $n$-by-$D$ data matrix and the corresponding $n$-by-$1$ outputs vector. We have seen that Tikhonov regularization defines an estimator considering the following  approximation\footnote{For the sake of simplicity, we are going to assume $\Xn^T\Xn$ to be invertible, but all the reasoning can be extended considering simply the pseudo-inverse of $\Xn$.
}

\begin{equation}\label{tikhofilter}
\lp \frac 1 n  \Xn^T\Xn +\la I \rp^{-1} \approx \lp \frac 1 n  \Xn^T\Xn\rp^{-1}.
\end{equation}
The regularization parameter $\la$ controls the condition number of such an approximation hence the (numerical) stability of the corresponding estimator. A natural question is whether other approximations can be considered to define different learning algorithms. Next we describe one such approximation.
Recall that for any $a\in (0,1)$ we have that
$$
\sum_{i=0}^\infty (1-a)^i=a^{-1}
$$
so that if we consider a truncated expansion we get
$$
\sum_{i=0}^{T-1} (1-a)^i\approx a^{-1}.
$$
If we now consider an invertible matrix  $A$ such that $\nor{A}<1$, then
we have that
$$
\sum_{i=0}^\infty (I-A)^i=A^{-1}.
$$
The above series is called the Neumann series. Following the reasoning in the scalar case,
an approximate inverse for $A$ can be defined considering a truncated series, that is
$$
\sum_{i=0}^{T-1} (I-A)^i\approx A^{-1}.
$$
In particular, if we take $A=\frac {2\gamma}{n} \Xn^T\Xn$, with $\gamma$ so that $\nor{A}<1$, then  we have
$$
\frac \gamma n \sum_{i=0}^{T-1}\lp I-\frac \gamma n \Xn^T\Xn\rp^i\approx
\lp \frac \gamma n  \Xn^T\Xn\rp^{-1}.
$$
The above expression can be contrasted to~\eqref{tikhofilter}. The parameter $\gamma$ is effectively chosen as a fixed constant, whereas the number of components controls the condition number and the quality of the approximation. In analogy with Tikhonov regularization we define an estimator as
\begin{equation}\label{LinLandClosedForm}
w_{T}= \frac{\gamma}{n}\sum_{i=0}^{T-1}\lp I-\frac \gamma n \Xn^T\Xn\rp^i\Xn^T\Yn.
\end{equation}
If we were to apply the above expression directly, we would incur in expensive computations. The discussion below shows that indeed we have an effective implementation as well as a
different, somewhat surprising, interpretation. Consider the iteration,
\begin{equation}\label{LinLand}
w_0=0;\quad w_{t+1}=w_t-\frac{\gamma}{n} \Xn^T(\Xn w_t-\Yn), \quad t=0, \dots, T-1,
\end{equation}
where the step-size is chosen to be a constant. The above iteration corresponds to $T$  steps of the gradient descent for  the empirical risk
$$
\En(w)=\frac{1}{2n} \nor{\Xn w-\Yn}_{\R^n}^2.
$$
The  intuition is that since the empirical risk is a proxy for the expected risk, considering the empirical gradient descent iteration  should provide a good solution. However,  if the iteration is let run too long the sequence will approach a minimizer of the expected risk, hence potentially an overfitting solution.
A good solution can be found by stopping at a suitable iteration $T$. The number of iterations is the only free parameter in the above procedure. This intuition is  grounded more rigorously in the observation that the iterate after $T$ steps is given exactly by~\eqref{LinLandClosedForm}.
Indeed, it is easy to see this by an induction argument.
The base case is easy to verify, and moreover, if we rewrite~\eqref{LinLand} as
$$
w_0=0;\quad w_{t+1}=\lp I- \frac{\gamma}{n} \Xn^T\Xn \rp w_t + \frac{\gamma}{n} \Xn^T \Yn, \quad t=0, \dots, T-1,
$$
then
\begin{eqnarray*}
w_{T}&=&
\lp I- \frac{\gamma}{n} \Xn^T\Xn \rp \frac{\gamma}{n}\sum_{i=0}^{T-2}\lp I-\frac \gamma n \Xn^T\Xn\rp^i\Xn^T\Yn+\frac{\gamma}{n}\Xn^T\Yn\\
&=&
\frac{\gamma}{n}\sum_{i=1}^{T-1}\lp I-\frac \gamma n \Xn^T\Xn\rp^i\Xn^T\Yn +\frac{\gamma}{n}\Xn^T\Yn\\
&=&
\frac{\gamma}{n}\sum_{i=0}^{T-1}\lp I-\frac \gamma n \Xn^T\Xn\rp^i\Xn^T\Yn.
\end{eqnarray*}
Then, for least squares, gradient descent can be seen to provide a stable solution to the empirical risk minimization problem, hence a good  approximate solution to the expected risk minimization problem.


The above reasoning directly applies to kernel defined by finite dictionaries. The extension to other kernels, is again straightforward using feature maps. To see this, first note that,
using again an induction argument, the iteration~\eqref{LinLand} can be written as
\begin{equation}\label{DulaLinLand}
w_t=\Xn^T c_t,\quad c_0=0,\quad c_{t+1}=c_t-\frac{2 \gamma}{n} (\Xn\Xn^T c_t-\Yn), \quad t=0, \dots, T-1.
\end{equation}
The above result is a form of the representer theorem for gradient descent which is useful when considering arbitrary kernels as can be seen from the following remark.
\begin{rem}[General Kernels]
Consider a   feature map $\Phi:\X\to \F$ with associated kernel
$K(x,x')=\scal{\Phi(x)}{\Phi(x')}_\F$. Follow the above derivation
where $\Xn$ is now replaced by the operator $\Phin:\F\to \R^n$ such that
$(\Phin w)_i=\scal{\Phi(x_i)}{w}_\F$, $i=1, \dots, n$ and  $w\in \F$, where we note that $\Phin\Phin^*=\Kn$.
Then, we can rewrite~\eqref{DulaLinLand} as
\begin{equation}\label{RepLand}
f_t(x)=\sum_{i=1}^n K(x_i,x)(c_t)_i
\end{equation}
with
\begin{equation}\label{DulaLinLandKer}
c_0=0\quad c_{t+1}=c_t-\frac{2 \gamma}{n} (\Kn c_t-\Yn), \quad t=0, \dots, T-1.
\end{equation}
The feature map is again only needed in the derivation while the end result only depends on computing the kernel function.
\end{rem}
We add a two more remarks.
\begin{rem}[Name Game]
Gradient Descent is a classical optimization method. When used with early stopping
to achieve regularization it is often called Landweber iteration and dates back to the fifties. In statistics it has been rediscovered recently and coined L2-Boosting, for an analogy with Boosting algorithms: each kernel function in~\eqref{RepLand} is seen as a weak {\em learner}
which is combined via~\eqref{RepLand} with weights which are iteratively found.
\end{rem}
The following remark regards modeling and computational aspects.
\begin{rem}[Computation \& Statistics]
When  compared to  Tikhonov regularization we see that the Landweber iteration is both an estimator and an actual algorithm. In this sense optimization and statistical aspects coincide in iterative regularization approaches such as Landweber iteration. A further important observation is that,  while gradient descent can be used to solve Tikhonov regularization we would be implicitly applying at the same time two forms of the same regularization principle, and we need to be aware of corresponding effects. For example choosing a large $\la$ might prevent the iteration to overfit even after many iterations or early stopping of the iteration might make the regularization effect of the norm penalty superfluous.
\end{rem}


==> chapters/statistical-learning-theory__copy_.tex <==
%\section{General Setting}

The field of machine learning studies algorithms and systems capable of extrapolating information and learning predictive models from data, rather than being specifically programmed to solve a given task.
These techniques are particularly useful for solving a wide range of tasks for which it is hard or unfeasible to define a comprehensive set of decision rules.
% - unlike classical approaches in Artificial Intelligence.
Examples of use are widespread, and include visual object recognition, speech recognition, control policy learning, fraud detection, dynamic pricing, and product ranking.
Machine learning
%(alone or in conjunction with other techniques included in a larger system) 
tackles this kind of problems by learning from examples.
It can be subdivided in the following main sub-fields:
\begin{itemize}
\item Supervised learning: The algorithm learns the mapping between inputs and desired outputs, based on a set of input-output pairs associated with the task, provided by a supervising entity. A performance measure (e.g. a loss function) is required.
\item Unsupervised learning: Data is made available to the learning algorithm, whose goal is to discover hidden structure in it. The provided examples do not include an output label. Main techniques falling in the definition include, among others: Clustering, feature learning, and dimensionality reduction techniques such as principal component analysis (PCA).
\item Reinforcement learning: The learning system has access to a dynamic environment, in which it has to perform a goal for which no supervision is provided. The actions applied to the environment result in a reward signal to be maximized in order to achieve the goal. Application examples include autonomous driving and general game playing.
\end{itemize}
In this work, the focus will be on supervised learning, in particular in the large-scale context.
In fact, when a significantly large number of data samples\footnote{We refer to input-output pairs as data points, samples or examples.} is available, learning algorithms can become too computationally expensive for execution.
This represents a relevant technological issue, hampering the way towards the applicability of machine learning methods.
For this reason, it is necessary to design novel large-scale learning algorithms capable of taking full advantage of the remarkable volume of data available today.
This unfolds many opportunities of scientific research, especially regarding the study of  the interplay between the statistical and computational properties\citep{bottou2007large} of these methods, and their generalization properties.
Throughout the work, we will analyze the statistical properties of supervised learning algorithms in the Statistical Learning Theory (SLT) \citep{cucker02onthe} framework, introduced next.

\section{Supervised Learning}

Supervised learning assumes to have access to a set of $n$ input-output pairs which are instances of the considered learning task.
This finite set of examples is called {\em training set}:
$$ 
S_n= \{(x_1,y_1),\dots,(x_n,y_n)\}.
$$
The objective of a supervised learning algorithm is {\em learning from examples}, that is by computing an estimator $f$, based on the training set, mapping \textit{previously unseen} inputs $x_{\text{new}}$ into the corresponding outputs $y_{\text{new}}$ (see Figure \ref{Fig:class_boundary}), as follows:
$$
%f(x_{\text{new}})\sim y_{\text{new}},
f: x_{\text{new}} \mapsto  y_{\text{new}}
$$
\begin{figure}[t]
\begin{center}
\includegraphics[width=3in]{figures/C2D3.pdf}
\end{center}
\caption{In binary classification, given examples (blue and red points) the problem is to learn a classifier (represented by the dashed line) correctly predicting the label of new input samples (white points).}
\label{Fig:class_boundary}
\end{figure}

The data are usually subject to {\em uncertainty} (e.g., due to noise).
Statistical learning models this by assuming the existence of an underlying probabilistic model for the data.\\
We will now more formally introduce the two fundamental concepts defining a learning task.
First, examples are drawn from the \textit{data space}, a probability space $\mathcal X \times \mathcal \Y$ with measure $\rho$.
$\mathcal \X$ is called \textit{input space}, while $\mathcal \Y$ is called \textit{output space} (see Figure \ref{Fig:functionalRelationship}).
\begin{figure}[t]
\begin{center}
\includegraphics[width=1.8in]{figures/domain.png}
\end{center}
\caption{Input and output space related by a functional relationship.}
\label{Fig:functionalRelationship}
\end{figure}
Secondly, a measurable {\em loss function} 
$$\ell: \mathcal Y \times \mathcal Y \to [0, \infty)$$
is defined to evaluate the quality of the predictions of the estimator.

On the basis of these key concepts, we can define the \textit{expected error} (more details are reported in Section~\ref{sec:expectedErr})
$${\cal E}(f) = \int_{\mathcal  X \times \mathcal Y} \ell(y, f(x)) d\rho(x,y).$$
The problem of learning is to find an estimator $f$ minimizing the expected error, that is solving
$$
\inf_{ f \in \mathcal F} {\cal E}(f),
$$ 
with $\rho$ fixed and unknown.
Here, $\mathcal F$ is the set of functions $f: \mathcal X \to \mathcal Y$ such that the expected risk ${\cal E}(f)$ is well defined.
%Since $\ell$ is measurable\footnote{$g: \mathcal X \to \R$ is measurable if, $\forall a \in \R$, the set $\{x \in \mathcal X:g(x)>a\}$ is measurable.} $f$ has to belong to the set of measurable functions, which is a very general one.
Access to $\rho$ is limited to a finite {\em training} set 
composed of samples identically and independently distributed (i. i. d.) according to $\rho$
$$S_n =\{ (x_1, y_1), \dots, (x_n, y_n)\} \sim \rho^n.$$
Since rho is known only via the training set $S_n$, finding an exact solution to the expected risk minimization is generally not possible.
One way to overcome this problem is to define an \textit{empirical error} measured on the available data to treat the learning problem in a computationally feasible way.
We first discuss in detail the concepts introduced above.

\section{Data Space}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The input/output examples belong to the {\em data space} $\mathcal{Z} = \mathcal{X} \times \mathcal{Y}$.
The \textit{input space} $\mathcal{X}$ can take several forms, depending on the specific learning problem. We report some of the most common cases:
\begin{itemize}
\item Linear spaces:
	\begin{itemize}
	\item Euclidean spaces: $\mathcal{X}\subseteq \R^d, \quad d \in \N$.
	\item Space of matrices: $\mathcal{X}\subseteq \R^{a \times b}, \quad a,b \in \N$.
%	\item Space of linear maps.
	\end{itemize}
\item Structured spaces:
	\begin{itemize}
	\item  Probability distributions: Given a finite set $\Omega$ of dimension $d$, we can consider as input space the space of all possible probability distributions over $\Omega$, which is $\mathcal X = \{x \in  \R^d_+ ~:~ \sum_{j=1}^d x^j=1\}$, $d\in \N$. This also holds more in general for any set  $\Omega$, even if not finite.
	\item Strings/Words: Consider an alphabet $\Sigma$ of symbols. The input space can be the space of all possible words composed of $p\in \N$, as follows: $\mathcal X=\Sigma^p$.
	\item $\mathcal X$ is a space of graphs.
	\end{itemize}
\end{itemize}


Similarly, the definition of output space $\mathcal{Y}$ results in several different categories of learning problems, some of the most common of which are:
\begin{itemize}
\item Linear spaces
	\begin{itemize}
	\item Regression: $\mathcal{Y}\subseteq \mathbb R$.
	\item Multi-output (multivariate) regression: $\mathcal{Y}\subseteq \mathbb R^T, T>1$.
	\item Functional regression: Outputs are functions, $\mathcal{Y}$ is a Hilbert space.
	\end{itemize}
\item Structured spaces
	\begin{itemize}
	\item $\mathcal{Y}$ is a space of probability distributions.
	\item $\mathcal{Y}$ is a space of strings.
	\item $\mathcal{Y}$ is a space graphs.
	\end{itemize}
\item Other spaces
	\begin{itemize}
	\item Binary classification: $\mathcal{Y}=\{-1,1\}$, or any pair of different numbers.
	\item Multi-category (multiclass) classification: Each example belongs to one among $T$ categories, $\mathcal{Y}=\{1,2, \dots, T\}, T \in \N$.
	\item Multilabel classification: Each example is associated to any subset of $T$ output categories, $\mathcal{Y}=2^{\{1,2, \dots, T\}}, T \in \N$.
	\end{itemize}
\end{itemize}
\begin{rem}[Multi-task Learning]
One of the most general supervised learning settings is called Multi-task Learning, for which $\mathcal Z = (\mathcal X_1,\mathcal Y_1) \times(\mathcal X_2,\mathcal Y_2) \times ... \times (\mathcal X_T,\mathcal Y_T) $ and the training set $S$ is composed of one training set $S_i$ for each task $i$ of the $T$ tasks: $S = {S_1, S_2, ..., S_T}, T\in \N$.
\end{rem}

\section{Probabilistic Data Model}
\label{sec:probDataModel}
In supervised learning, in order to estimate an input/output relation, we assume that a model expressing this relationship exists. In SLT, the assumed model is probabilistic, in the sense that the data samples constituting the training and the test sets are assumed to be sampled independently from the same fixed and unknown data distribution $\rho(x,y)$\footnote{In this case, we say that data samples are independent and identically distributed (i. i. d. assumption).}
 on the data space $\mathcal{Z}$.
Thus, $\rho$ encodes the uncertainty in the data and in the learning task, for instance caused by noise, partial information or quantization.
By also assuming that $\rho(x,y)$ can be factorized as
$$\rho(x,y)=\rho_{\mathcal{X}}(x)\rho(y|x) \quad \forall (x,y) \in \mathcal{Z},$$
the various sources of uncertainty can be separated.
In particular, the marginal distribution $\rho_{\mathcal{X}}(x)$ models the uncertainty in the sampling of the input points.
Instead, $\rho(y|x)$ is the conditional distribution modeling the {\em non deterministic} input-output mapping, as shown in Figure \ref{Fig:Conditional}.
\begin{figure}[t]
\begin{center}
\includegraphics[width=2.8in]{figures/insiemi.pdf}
\end{center}
\caption{Given an input $x$,  the yellow area is the support of its associated distribution of possible outputs $\rho(y|x)$. The green area represents the support of the distribution of all possible outputs $\rho(y)$.}
\label{Fig:Conditional}
\end{figure}
We now consider two instances of data model, associated with regression and classification.
\begin{ex}[Fixed and Random Design Regression]
In statistics, the commonly assumed data model for regression is the following,
$$y_i=f^*(x_i)+\epsilon_i,$$
where $\mathcal{X} = \{x_1,  x_2, ..., x_n\}$ is a deterministic discrete set of inputs, $f^*$ is a fixed unknown function and $\epsilon$ is random noise.
For example, $f^*$ could be a linear function $f^*(x)=x^\top w^*$ with $w^*\in \R^d$, and the $\epsilon$ component could be Gaussian noise, distributed according to ${\mathcal N}(0,\sigma )$, $\sigma\in [0,\infty)$.
The aforementioned model is named \textit{fixed design regression}, since $\mathcal{X}$ is fixed and deterministic.
By contrast, in SLT the so-called \textit{random design} setting is often considered, according to which the training samples are not given a-priori, but according to a probability distribution $\rho_{\mathcal X}$ (for example, uniformly at random).
See Figure \ref{Fig:Regression} for an example.
\end{ex}
\begin{figure}[t]
\begin{center}
\includegraphics[width=2.8in]{figures/regression.pdf}
\end{center}
\caption{Fixed unknown linear function $f^*$ and noisy examples sampled from the $y=f^*(x)+\epsilon$ model.}
\label{Fig:Regression}
\end{figure}

\begin{ex}[Binary classification]
In binary classification, input-output samples are sampled randomly according to a distribution $\rho$ over $\X \times \{-1, 1\}$.
In a simple example of binary classification problem, $\rho$ is a mixture of two Gaussians, each corresponding to a class, $\rho(x,y) =  \rho(x|y=-1) + \rho(x|y=-1)$, with
$$\rho(x|y=-1)=\frac 1 c {\mathcal N}(-1,\sigma_- ), \, \sigma_-\in [0,\infty)$$ 
$$\rho(x|y=1)=\frac 1 c {\mathcal N}(+1,\sigma_+), \, \sigma_+\in [0,\infty)$$
where $c \in \R$ is a suitable normalization factor such that $\rho(x,y)$ is a probability distribution, that is s. t. $\int \rho(x,y) dx dy = 1$.
An example dataset drawn according to the aforementioned $\rho(x,y)$ is shown in Figure \ref{Fig:Classification}
\end{ex}
\begin{figure}[h!]
\begin{center}
\includegraphics[width=2.8in]{figures/classification.pdf}
\end{center}
\caption{2-D example of a dataset sampled from a mixed Gaussian distribution. Samples of the yellow class are realizations of a Gaussian centered at $(-1,0)$, while samples of the blue class are realizations of a Gaussian centered at $(+1,0)$. Both Gaussians have standard deviation $\sigma = 0.6$.}
\label{Fig:Classification}
\end{figure}

 
\section{Loss Function}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We have seen that the problem of learning an estimator amounts to finding a function $f$ ``best" approximating the underlying input-output relationship.
To do so, we need a measure of the predictive accuracy of the learned estimator with reference to the specific learning task in exam.
In particular, the most natural way to do so is to define a point-wise {\em loss function} 
$$
\ell:\mathcal{Y}\times \mathcal{Y}\to [0,\infty),
$$
measuring the loss $\ell(y, f(x))$ the learning system undergoes by predicting $f(x)$ instead of the actual output $y$.
%The loss function choice is intimately linked to the specific learning task in exam.
For instance, typical losses for regression problems differ from the ones used for classification.
%Disregarding the most exotic cases, loss functions are usually symmetric.
We will now review some of the most usual loss functions.\\
Loss functions for regression
%fall under following definition $\ell:\mathcal{Y}\times \mathcal{\R}\to [0,\infty)$, and 
usually depend on the deviation $y-a$ between the real output $y$ and the predicted value $a = f(x)$.
\begin{itemize}
	\item Square loss: It is the most commonly employed loss function for regression, defined as $\ell(y,a) = (y-a)^2$, with $a,b \in \mathcal Y$.
	\item Absolute loss: $\ell(y,a) = | y-a |$
	\item $\epsilon$-insensitive loss: $\ell(y,a) = max\{| y-a |- \epsilon,0\}$, with $\epsilon \in (0,+\infty)$. It is used in Support Vector Machines (SVMs) for regression \citep{smola1997support}.
\end{itemize}
Loss functions for regression are shown in Figure \ref{fig:regressionloss}.
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{./figures/regr-loss.pdf}
\caption{Loss functions for regression.}
\label{fig:regressionloss}
\end{figure}
Loss functions for classification: For the sake of simplicity, we consider the setting in which $\mathcal Y = \{+1,-1\}$.
\begin{itemize}
\item Misclassification loss (0-1 loss, counting loss): It is probably the most natural choice for measuring the accuracy of a classifier.
It assigns a cost $1$ if the predicted label is incorrect, and $0$ otherwise. 
It can be defined as $\ell(y,a) = \ind_{y \neq a}$, where $\ind_{(\cdot)}$ is the indicator function, $y$ is the real output associated to the input $x$, and $a = \text{sign}(f(x))$ is the output label predicted by the learned estimator $f$.
\item Surrogate losses: The 0-1 loss is non-convex and makes optimization hard.
To overcome this issue, convex \textit{surrogate loss functions} acting as convex relaxations of the 0-1 loss are introduced.
To introduce them, we consider the real-valued prediction $a = f(x)$, without taking the sign.
Thus, given a pair $(x,y)$ and an estimator $f$, we define the quantity $ya$, called \textit{margin}.
Surrogate losses are often defined in terms of margin: $\ell(y,a) = \ell(ya)$.
We report the most commonly used ones below:
	\begin{itemize}
	\item Hinge loss: Used in Support Vector Machines (SVM) for classification, it is defined as $\ell(y,a) = |1-ya|_+ = max\{ 1-ya, 0 \}$.
	\item Exponential loss: $\ell(y,a) = e^{-ya}$, used in Boosgting algorithms.
	\item Logistic loss: $\ell(y,a) = log(1+e^{-ya})$, used in logistic regression.
	\item Square loss: It can be used also for classification, and it can be written in terms of margin as $\ell(y,a) = (y-a)^2 = (1-ya)^2$.
	\end{itemize}
\end{itemize}
See Figure \ref{fig:classloss} for a pictorial representation of the aforementioned loss functions for classification in terms of margin $ya$.
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{./figures/class-loss.pdf}
\caption{Margin-based loss functions for classification.}
\label{fig:classloss}
\end{figure}



\section{Expected Error}
\label{sec:expectedErr}
The loss function $\ell$, alone, is not enough for quantify how well an estimator performs on any possible future data sample drawn from $\rho$.
To this end, we first define the \textit{expected error} (also {\em expected risk} or \textit{expected loss}) of an estimator $f$ given a loss $\ell$ as
\begin{equation}\label{eq:expectedError}
{\mathcal E}(f)=\int_{\mathcal  X \times \mathcal Y} \ell(y, f(x)) d\rho(x,y),
\end{equation}
which expresses the average loss the estimator is expected to incur in on samples drawn according to $\rho$.
Hence, in the SLT framework the ``best"  possible estimator is the {\em target function} $f^*:\mathcal X\to \mathcal Y$ minimizing ${\mathcal E}(f)$,
$$
\inf_{f \in \mathcal F}  {\mathcal E}(f),
$$
where $\mathcal F$ is named \textit{target space} and is the space of functions for which ${\mathcal E}(f)$ is well-defined.
Note that different loss functions yield different target functions, as reported in Appendix~\ref{app:lossTarget}.
It is essential to note that this minimization cannot be computed in general, because the data distribution $\rho$ is not available.
The objective of a learning algorithm is to find an estimator $f$ as close as possible to $f^*$ and behaving well on unseen data, despite having access to just a finite realization $S_n \sim \rho^n$, the training set.
An algorithm fulfilling this criterion is said to \textit{generalize well}, which is the cornerstone concept of SLT --- and machine learning in general.
% --- mostly differentiating it from stand-alone Mathematical Optimization.
%\begin{rem}[Decision Surface/Boundary]
%In classification we often visualize the so called decision boundary (or surface) of a classification solution $f$. 
%The decision boundary is  the  level set of points $x$ for which $f(x)=0$.
%\end{rem}



\section{Generalization Error Bound}
A learning algorithm $\mathcal{A}$ can be thought of as a mapping $\mathcal{A}: S_n \mapsto \fn$ from the the training set $S_n$ to the associated estimator $\fn$.
To introduce the concepts of generalization and consistency, we assume that $\mathcal{A}$ is deterministic, even if this assumption can be relaxed, as we will see in the following chapters.
Here, the only source of uncertainty is therefore due to stochasticity in the data, modeled by $\rho$.

We have seen that the target function associated to a learning problem is the one minimizing the expected risk.
A good learning algorithm is able to find an estimator $\fn$ yielding an expected error as close as possible to the one of the target function.
%In loose terms, the qualitative objective is to have
%$$
%\EE(\fn)\approx \EE(f^*) = \inf_{f\in\mathcal F} \EE(f).
%$$
However, to perform a more precise analysis of a learning algorithm we need to quantify this behavior, considering that the learned estimator $\fn$ depends on the training set $S_n$.
%%% Learning rate
A widely studied property of learning algorithms is the \textit{generalization error bound}, which describes a bound on the error with probability $1-\delta$.
More formally, given a distribution $\rho$,
$\forall \delta \in[0,1], n >0$, there exists a function $\epsilon(\delta,n)$, called \textit{learning rate} (or \textit{learning error}), such that,
\begin{equation}\label{eq:learningRate}
\P\left( \EE(\fn)-\inf_{f\in\mathcal F} \EE(f)\le \epsilon(\delta,n) \rp \ge 1- \delta.
\end{equation}

%For instance, given a training set size $n$, we can study the probability that $\EE(\fn) -\EE(f^*)$ is larger than a threshold $\epsilon \in \R^+$, which is
%$$
% \P\lp\EE(\fn)-\inf_{f\in\mathcal F} \EE(f)>\epsilon\rp.
%$$
%Intuitively, a desirable property would be for this quantity to go to zero as $n$ goes to infinity.
%Thus, we introduce the \textit{consistency} property.
%Given a data distribution $\rho$, a learning algorithm is consistent if
%\begin{equation}\label{ucons}
%\lim_{n\to \infty} \P\lp\EE(\fn)-\inf_{f\in\mathcal F} \EE(f)>\epsilon\rp=0, \quad \forall \epsilon>0.
%\end{equation}
%The algorithm is said to be \textit{universally consistent} if \eqref{ucons} holds for any distribution $\rho$ on the data space $\mathcal Z$.
%The objective of supervised learning can be formalized in terms of the consistency property as follows:
%\begin{quote}
%{\em Given a sample of input/output pairs, i.i.d. with respect to a fixed unknown distribution, and a loss function, the goal of supervised learning is to find a universally consistent algorithm.}
%\end{quote}
%Universal consistency allows us to study the asymptotic properties of a learning algorithm.
%%Hence, we introduce {\em uniform universal consistency}, a stronger property characterizing the behavior of the estimator for a finite number of samples.
%%\begin{equation}\label{uucons}
%%\lim_{n\to \infty} \sup_{\rho} \P\left( \EE(\fn)-\inf_{f\in\mathcal F} \EE(f)>\epsilon\rp=0, \quad \forall \epsilon>0.
%%\end{equation}
%The universal consistency property~\eqref{ucons} can be rewritten as a \textit{finite sample bound}, yielding information about the minimum number of  samples needed by the algorithm to reduce the quantity $\EE(\fn) -\EE(f^*)$ below a certain threshold $\epsilon$ with high probability.
%More formally, given a distribution $\rho$,
%$\forall \delta, \epsilon >0$, $\exists n_\rho(\epsilon,\delta)$ such that, if $n\ge n_\rho(\epsilon,\delta)$, then
%$$
%\P\lp \EE(\fn)-\inf_{f\in\mathcal F} \EE(f)\ge \epsilon\rp\le \delta.
%$$
%Here, $n_\rho(\epsilon,\delta)$ is called \textit{sample complexity} and in general depends on $\rho$.\\
%%Similarly, by rewriting the  \textit{uniform} universal consistency property~\eqref{uucons} we obtain a comparable definition in which the resulting sample complexity $n(\epsilon,\delta)$ does not depend on $\rho$.
%Similarly, the \textit{learning rate} (or \textit{learning error}) is defined as the function $\epsilon(\delta,n)$ such that, for $\sigma > 0$,
%\begin{equation}\label{eq:learningRate}
%\P\left( \EE(\fn)-\inf_{f\in\mathcal F} \EE(f)\le \epsilon(\delta,n) \rp \ge 1- \delta.
%\end{equation}

%\begin{rem}[Sample Complexity, Error Bounds and Tail Estimates]
%The function $n(\delta,\epsilon)$ is often invertible with respect to both $\epsilon$ and $\delta$, so that we can get some equivalent formulations. 
%For example, solving with respect to $\epsilon$ we obtain,
%$$
%\P\left( \EE(\fn)-\inf_{f\in\mathcal F} \EE(f)\le \epsilon(\delta,n) \rp \ge 1- \delta
%$$
%and the function $\epsilon(\delta,n)$ is called the learning rate or learning error.
%If we solve with respect to $\delta$ we obtain,
%$$
%\P\left( \EE(\fn)-\inf_{f\in\mathcal F} \EE(f)>\epsilon\rp\le \delta(n,\epsilon).
%$$
%where $\delta(n,\epsilon)$ is a tail estimate.
%\end{rem}


%Foundational results in statistical learning theory (see later chapters), show that uniform universal consistency is in fact impossible. If we are interested in quantifying the finite sample properties of an algorithm we have to weaken the requests in~\eqref{uucons}. One possibility is to consider a restricted class of distributions $\Theta$, and
%\begin{equation}\label{prior_cons}
%\lim_{n\to \infty} \sup_{\rho\in \Theta} \P\left( \EE(\hat{f})-\inf_{f\in\mathcal F} \EE(f)>\epsilon\rp=0, \quad \forall \epsilon>0.
%\end{equation}
%Another possibility is to replace the target space with some smaller set of functions $\hh\subset {\mathcal F}$, that is
%\begin{equation}\label{dfree_cons}
%\lim_{n\to \infty} \sup_{\rho} \P\left( \EE(\hat{f})-\inf_{f\in\hh} \EE(f)>\epsilon\rp=0, \quad \forall \epsilon>0.
%\end{equation}
%Note that in the first case the sample complexity becomes $n_\Theta(\epsilon,\delta)$ and describes a property of class $\Theta$, whereas in the second case it becomes $n_\hh(\epsilon,\delta)$ and describes a property of class $\hh$.


\section{Empirical Risk Minimization \& Hypotheses Space} 
\label{sec:ERM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A good learning algorithm is able to find an estimator $f$ approximating the target function $f^*$.
From the computational viewpoint, though, the minimization of the expected risk yielding $f^*$,
$$
\inf_{f \in \mathcal{F}} \EE(f),
$$
is unfeasible, since $\rho$ is unknown and the algorithm can only access a finite training set $S_n$.
%Secondly, the target space $\mathcal{F}$ is very general and not accessible.
An effective approach to learning algorithm design in this setting is to minimize the error on the finite training set instead of the whole distribution.
To this end, given a loss $\ell$ we define the {\em empirical risk (or empirical error)}
$$
\EM(f)=\frac 1 n \sum_{i=1}^n \ell(y_i, f(x_i)),
$$
acting as a proxy for the expected error defined in~\eqref{eq:expectedError}.
%$$
%{\mathcal E}(f)={\mathbb E}[\ell(y,f(x))]=\int \rho(x,y)\ell(y,f(x))dxdy,
%$$
%Secondly, it is necessary to replace the space $\mathcal F$ with one we have access to.
In practice, to turn the above idea into an actual algorithm we need to select a suitable hypotheses space  $\mathcal H \subset \mathcal F$ of candidate estimators, such that $\EM(f)$ is well defined $\forall f \in \mathcal{H}$.
The hypotheses space should be such that computations are feasible and, at the same time, it should be {\em rich} enough to approximate $f^*$.
%since the complexity of the problem is not known a priori. 
%On the other hand, we would like to be able to control the complexity of the solution 
%to avoid instability, hence overfitting.
%The simplest example of hypotheses space 
%is  the  space of linear functions, that is 
%\begin{equation}\label{linearFunctionsSpace}
%\mathcal H=\{f:\mathbb R^d\to \mathbb R~:~ \exists w\in \ \mathbb R^d ~\text{such that}~ f(x)=x^\top w, ~\forall x \in \mathbb R^d\}.
%\end{equation}
%Each function $f$ is defined by a vector $w$ and we let $f_w(x)=x^\top w$.
%We will see how to define richer hypotheses spaces in Chapter \ref{Chap:kernelMethods}.
To sum up, the ERM problem can be written as
\begin{equation}\label{HExpErrMin}
\inf_{f\in \hh} \EM(f),
\end{equation}


%We have also seen how we can vastly extend 
%the class of functions we can consider by introducing a feature map 
%$$\Phi:\mathbb R^d\to \mathbb R^p,$$ where typically 
%$p\gg d$, and considering functions of the form $f_w(x)=\Phi(x)^Tw$. We have also seen how this model can be pushed further
%considering so called reproducing kernels
%$$
%K:\mathbb R^d\times \mathbb R^d\to \mathbb R
%$$
%that are symmetric and positive definite functions, implicitly defining a feature map via the equation
%$$
%\Phi(x)^T\Phi(x')=K(x,x').
%$$


\section{Overfitting and Regularization} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
Ideally, an estimator $\fn$ should  {\em mimic}  the target function $f^*$, in the sense that its expected error should be close to the one of $f^*$ as $n \rightarrow \infty$.
%${\mathcal E}(\fn)\approx {\mathcal E}(f^*)$.
The latter requirement needs some care, since  $\fn$ depends on the training set $S_n$ and hence is random.
As we have seen in \eqref{eq:learningRate}, one possibility is to require an algorithm to have a good learning rate.
%As we have seen, one possibility is to require an algorithm to be good in {\em expectation}, in the sense that  
%$${\mathbb E}_S [ {\mathcal E}(\fn)-{\mathcal E}(f^*) ],$$
%is small.
Given a rich enough hypotheses space $\hh$, 
%such that
%$$
%\inf_{f\in \hh} \EE(f)\approx \inf_{f\in \mathcal F} \EE(f),
%$$
a good learning algorithm should be able to describe well (fit) the data
and at the same time 
disregard noise. 
%%% Variance
Indeed, a key to ensure good generalization is to avoid \textit{overfitting}, that characterizes estimators which are highly dependent on the training data.
%, possibly with a low error on the training set and yet a large error on future data.
In other words, the empirical risk can become very small, while the expected risk remains large.
This can happen if $\hh$ is too rich, thus making the model ``learn the noise'' in the training data.
In this case, the estimator is said to have high \textit{variance}.
%$$
%\inf_{f\in \hh} \EM(f)\not\approx \inf_{f\in \hh} \EE(f).
%$$
%%% BIAS
On the other hand, if $\hh$ is too simple the estimator is less dependent on the training data and thus more robust to noise, but $\hh$ may not be rich enough to approximate well the target function $f^*$.
This yields both high empirical and high expected risks.
%%% REGULARIZATION
\textit{Regularization} is  a general class of techniques that allow to restore stability and ensure generalization.
It considers a sequence of hypotheses spaces $\hh_\la$, parameterized by a \textit{regularization parameter}$\la$, with
$$
\lim_{\la \rightarrow 0} \hh_{\la} = \F.
$$
One possible method for controlling the size of the hypothesis space via a parameter $\la$ is \textit{Tikhonov regularization} \citep{TikhonovOriginal}.
This method adds a so-called \textit{regularizer} to the empirical risk minimization problem in \eqref{HExpErrMin}, that controls the size of $\hh_{\la}$.
A regularizer is a functional $R:\hh\to [0,\infty)$ that penalizes estimators which are too ``{\em complex}".
In this case we could replace~\eqref{HExpErrMin} by
\begin{equation}\label{RExpErrMin}
\inf_{f\in \hh} \EM(f) +\lambda R(f),
\end{equation}
for some \textit{regularization parameter} $\lambda>0$.
%We broadly refer to this class of approaches as regularization algorithms, and their study in large-scale scenarios is our main topic of discussion.
%If the hypotheses space is too rich, solely minimizing the empirical risk is not sufficient to ensure a generalizing solution, because it would lead to estimators which are highly dependent on the (noisy) training data and could overfit.
%
%\section{Tikhonov Regularization and Representer Theorem} 
%\label{sec:tikhonovReg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%We consider the following {\em Tikhonov} regularization scheme,
%\begin{equation}\label{eq:Tikho}
%\min_{w\in \mathbb R^d}
%\EM(f_w)
%%\frac 1 n \sum_{i=1}^n \ell(y_i, f_w(x_i))
%+\lambda \|w\|^2.
%\end{equation}
%The above scheme describes a large class of methods sometimes called Regularization Networks. 
%The term  $ \|w\|^2$ is called regularizer and  controls the stability  of the solution. The parameter 
%$\lambda$ balances the error term and the regularizer, as we will discuss later. 
%
%Different classes of methods are induced by the choice of different loss functions.
%In the following, we will see common aspects and differences in considering different loss functions.
%
%There is no general computational scheme to solve problems of the form~\eqref{eq:Tikho}, and
%the actual solution for each algorithm depends on the considered loss function. 
%However,  we show next that for linear functions the solution of problem~\eqref{eq:Tikho} can always be written as
%\begin{equation}\label{eq:repre}
%w=X^\top \alpha, \quad f(x)=\sum_{i=1}^n x^\top x_i \alpha_i
%\end{equation}
%where $X$ is the $n \times d$ data matrix and $\alpha=(\alpha_1, \dots, \alpha_n)$. 
%This  allows on the one hand to reduce computational complexity when $n\ll d$, or $n\ll p$ in the case of a feature map. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Representer Theorem for General Loss Functions}
%
%
%Here we discuss the general proof of the representer theorem for loss functions other than the square loss.
%
%
%\begin{itemize}
%\item The  vectors of the form~\eqref{eq:repre} form a linear subspace $\widehat W$ of $\mathbb R^d$. 
%Hence, for every $w\in  \mathbb R^d$ we have the decomposition $w=\widehat w + \widehat w^\perp$, where $\widehat w \in \widehat W$ and $\widehat w^\perp$ belongs to the space 
%${\widehat W}^\perp$ of vectors orthogonal to those in $\widehat W$ , i.e. 
%\begin{equation}\label{ortho}
%\widehat w^\top \widehat w^\perp=0.
%\end{equation}
%\item The following is the key observation: for all $i=1, \dots, n$ $x_i\in \widehat W$, so that 
%$$
%f_w(x_i)=x_i^\top w=x_i^\top (\widehat w+\widehat w^\perp)=x_i^\top \widehat w.
%$$
%It follows that the empirical error depends only on $\widehat w$.
%\item For the regularizer we have 
%$$
%\|w\|^2=\|\widehat w+\widehat w^\perp\|^2=\|\widehat w\|^2+\|\widehat w^\perp\|^2,
%$$
%because of~\eqref{ortho}.
%Clearly, the above expression is minimized if we take $\widehat w ^\perp=0$.
%\end{itemize}
%The theorem is hence proved, the first term in~\eqref{eq:Tikho} depends only on vector of the form~\eqref{eq:repre} and the same form is the best to minimize the second term
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Bias Variance Decomposition and Model Selection}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%Here we study  the question of how to choose the number of neighbors $K$ in KNN: is there an optimal choice of $K$? Can it be computed in practice? 
%Towards answering these questions we investigate theoretically the  question  of how $K$ affects the performance of the KNN algorithm. 
%Most of the ideas and results in the following  generalize to  a large class of learning algorithms beyond KNN. 
%Indeed, many (most) learning algorithms depend on one or more parameter controlling their performances.
%
%Recall that the KNN algorithm defines an estimator as 
%$$
%\hat f _K(x)= \frac 1 K \sum_{\ell \in \Lambda_K(x)} y_\ell,
%$$
%where $\Lambda_K(x)$ are the indices of the $K$ input points closest to $x$. 
%
At this point, a natural question is whether an optimal regularization parameter in terms of learning algorithm performance exists, and, if so, how it can be computed in practice.
%We examine the case of Tikhonov regularization with the square loss, but the analysis holds for a broad variety of regularized learning algorithms.
%The goal is to choose a regularization parameter $\lambda$ that minimizes the expected error 
%$$
%\EE(\hat f _\lambda) = {\mathbb E} _S {\mathbb E} _{x,y} (y-\hat f _\lambda(x))^2,
%$$
%for
%\begin{equation}%\label{RExpErrMin}
%$$
%\hat f _\lambda = \text{arg} \inf_{f\in \hh} \hat \EE(f) +\lambda R(f).
%$$
%\end{equation}
We next characterize the corresponding minimization problem to uncover one of the most 
fundamental aspects of machine learning.
%For the sake of simplicity, we consider a regression model 
%$$
%y_i=f_*(x_i)+\delta_i, \quad {\mathbb E} \delta_i=0, {\mathbb E} \delta_i^2=\sigma^2 \quad i=1, \dots, n .
%$$
As we saw in the previous sections, the generalization  performance of a learning algorithm 
%can be expressed in terms of the so-called \textit{excess risk}
is as much high as
% the \textit{excess risk}
\begin{equation}\label{Perf}
%\EE(\hat f _\lambda) - \EE(f ^*) =  
\EE(\fn _\lambda) -  \inf_{ \F} \EE(f),
\end{equation}
is low, with 
$$
\fn _\lambda = \arginf_{f\in \hh} \EM(f) +\lambda R(f).
$$
In particular, we will use the squared norm in $\hh$ as a regularizer, obtaining
\begin{equation}\label{eq:TikhoII}
\fn _\lambda = \arginf_{f\in \hh} \EM(f) +\lambda \|f\|_\hh^2,
\end{equation}
with $\|f\|_\hh^2 = \langle f,f \rangle_{\hh}$.
To get an insight on how to choose $\lambda$, we analyze theoretically how this choice influences performance. % the excess risk.
For a fixed $\la$, we can decompose \eqref{Perf} as
\begin{equation}\label{BiasVarianceDecomp}
 \EE(\fn _\lambda)- \inf_{ \F} \EE(f)
 =  
\underbrace{ \EE(\fn _\lambda)- \inf_{ \hh_\la} \EE(f) }_{Variance}
 + 
\underbrace{  \inf_{ \hh_\la} \EE(f)- \inf_{ \F} \EE(f) }_{Bias}.
\end{equation}
%The above scheme can be seen as a form of regularization.
Indeed, on the one hand we introduce a {\em variance} term to control the complexity of the hypotheses space.
On the other hand, we allow the class complexity to grow to reduce the \textit{bias} term.\\
Specifically, by bias we mean the deviation
$$ \inf_{ \hh_\la} \EE(f)- \inf_{ \F} \EE(f).$$
This is often called the {\em approximation error} and does not depend on the data but only on how well the class $\hh_\la$ ``approximates'' $\F$.
There are many instances of the above setting in which it is possible to design
regularization schemes so that the approximation error \textit{decreases for decreasing} $\la$.
In fact, in such schemes a small $\la$ corresponds to a reduced penalization of rich function classes.\\
In contrast, the term 
$$\EE(\fn_\lambda)- \inf_{ \hh_\la} \EE(f)$$ 
is called {\em sample}, or {\em estimation error}, or simply the \textit{variance} term.
It is data dependent and stochastic, and measures the variability of the output of the algorithm, for a given complexity, with respect to an idealized algorithm having access to all the data.
In most regularized learning algorithms a small $\la$ corresponds to a complex model which is more sensitive to data stochasticity, thus leading to a larger variance term.\\
%Once we consider a set of candidate regularized solutions for a given learning problem, as described above, the question arises about which solution should be selected.
%%We describe this question next.
%In theory, if we had access to bounds for the sample and approximation error of an algorithm we could simply optimize the bound to select a specific level of complexity, hence an element of the sequence (e.g., an optimal $\la$).
%More formally, if we have that
%\begin{equation}\label{OptBound}
%\begin{gathered}
% \EE(\fn _\lambda)- \inf_{ \F} \EE(f)=\\
%   \EE(\fn _\lambda)- \inf_{ \hh_\la} \EE(f)+ \inf_{ \hh_\la} \EE(f)- \inf_{ \F} \EE(f)\le S(\la,n)+A(\la),
%\end{gathered}
%\end{equation}
%where $S(\la,n)$ and $A(\la)$ are the upper bounds for the sample and approximation errors, respectively,
%and a set of candidate regularization parameters $\Lambda$ is provided,
%then a parameter choice can be defined as
%\begin{equation}\label{lambdaZero}
%\la_0=  \min_{\la \in \Lambda} \lc S(\la,n)+A(\la)\rc.
%\end{equation}
%A corresponding rate will be given by
%\begin{equation}
% \EE(\fn _{\lambda_0})- \inf_{ \F} \EE(f).
%\end{equation}
%To ensure that the above approach makes sense, we need the bound to be sufficiently \textit{tight}.
%Ideally, we would like to have a matching lower bound, that is to know that
%$$
% \EE(\fn _\lambda)- \inf_{ \F} \EE(f)\ge c\lp S(\la,n)+A(\la)\rp
%$$
%for some numerical constant $c\in \R$.
%In this case the bound~\eqref{OptBound} is called {\em optimal}.




\section{Bias Variance Trade-off and Cross-validation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[t!]
\begin{center}
\includegraphics[width=2.7in]{figures/biasvariance.png}
\end{center}
\caption{The Bias-variance trade-off. In Tikhonov regularization the parameter $\la$ controls the model's complexity. A small $\la$ yields high complexity, and vice-versa.}\label{Fig:BiasVariance}
\end{figure}

In this section we will briefly discuss some practical considerations regarding the regularization parameter choice  for regularized learning algorithms ``\textit{\`a la Tikhonov}''.
As previously introduced, variance decreases with $\la$, while bias increases with $\la$.
A larger bias is preferred when training samples are few and/or noisy to achieve a better control of the variance, while it can be decreased for larger datasets.
For any given training set, the best choice of $\lambda$ would be the one guaranteeing the optimal trade-off between bias and variance (that is the value minimizing their sum), as shown in Figure \ref{Fig:BiasVariance}.
However, the theoretical analysis is not directly useful in practice since the data distribution,
 hence the expected loss, is not accessible.
 In practice, data driven procedures are used to find a proxy for the expected loss, the simplest of which is called \textit{hold-out cross-validation}. 
 Part of the training set is held-out and used to compute a (hold-out) error acting as a proxy of the expected error.
  An empirical bias-variance trade-off is achieved choosing the value of $\la$ achieving the minimum hold-out error.
  When data are scarce, the hold-out procedure, based on a simple "two ways split" of the training set, might be unstable.
  In this case, so called $V$-fold cross validation 
 is preferred, which is based on multiple data splitting. More precisely, the data are divided in $V \in [2,...,n] $ 
 (non overlapping) sets.
 Each set is held-out and used to compute a hold-out error which is eventually averaged to obtain the final $V$-fold  cross-validation error.
 The extreme case where $V=n$ is called \textit{leave-one-out} cross-validation.\\
%We briefly discuss more formally the hold-out cross-validation procedure.
%Consider a training set $S$, and further assume a hold-out set $S'$, both drawn i.i.d. according to the same data distribution $\rho$.
%Given a sequence of regularized solutions $\fn_\la$, the idea is to consider the parameter choice
%$$
%\hat \la = \argmin_{\la \in \Lambda} \En'(\fn_\la),
%$$
%where $\Lambda$ is a finite set obtained by discretizing the possible values of $\la$ and $\En'$ the empirical risk on $S'$. Note that we can view the above procedure as a form of empirical risk minimization over a finite set.\\
%Then, from  previous results we might expect that  it should be possible to control
%%$$
%%\EE(\fn^{\hat \la}) - \min_{\la \in \Lambda} \EE(f^\la)
%%$$
%$$
%\EE(\fn_{\hat \la}) - \min_{\la \in \Lambda} \EE(f_\la),
%$$
%where we assumed that $\EE(f_\la) =\min_{f\in \hh_\la}\EE(f)$,
%by means of an upper bound $\eta(n)$.
%If $\eta(n)$ were available, by simply adding and subtracting $\inf_{f \in \F} \EE(f)$ we would obtain
%$$
% \EE(\fn_{\hat \la}) - \inf_{f \in \F} \EE(f) \le \min_{\la \in \Lambda} \EE(f_\la) - \inf_{f \in \F} \EE(f) + \eta(n).
%$$
%If we assume the effect of the discretization of $\lambda$ to be negligible, we have
%$$
% \EE(\fn_{\hat \la}) - \inf_{f \in \F} \EE (f) \le \EE(\fn_{\la_0})- \inf_{f \in \F} \EE(f) +\eta(n),
%$$
%with $\lambda_0$ as defined in \eqref{lambdaZero}.
%%where $\lambda_0$ 
%As a result, generalization performance can be controlled in practice via hold-out cross-validation.


\section{Regularized Least Squares}
\label{sec:RLS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we introduce Regularized Least Squares (RLS), a learning algorithm based on Tikhonov regularization employing the square loss.\\
The learning algorithm is defined as
\begin{equation}\label{eq:Tikhorls}
\min_{w\in \mathbb R^d}
%\hat {\mathcal E}(f_w)
\frac 1 n \sum_{i=1}^n (y_i-  w^\top x_i)^2
+\lambda w^\top w,\quad  \lambda \ge 0,
\end{equation}
considering as hypotheses space the class of linear functions, that is 
\begin{equation}\label{linearFunctionsSpace}
\mathcal H=\{f:\mathbb R^d\to \mathbb R~:~ \exists w\in \ \mathbb R^d ~\text{such that}~ f(x)=x^\top w, ~\forall x \in \mathbb R^d\}.
\end{equation}
Each function $f$ is defined by a vector $w$ and we let $f_w(x)=x^\top w$.
A motivation for considering the above scheme is to view  the empirical risk 
$$
\En(f_w) = 
\frac 1 n \sum_{i=1}^n (y_i-  w^\top x_i)^2,
$$
with $f_w(x) = w^\top x$, as a proxy for the expected risk
$$
\EE(f_w) =  
\int \rho(x,y)(y-  w^\top x)^2 dxdy,
$$
which is not computable.
%We have implicitly chosen the space of possible solutions, called the hypotheses space, to be
% the  space of linear functions, that is 
%$$
%H=\{f:\mathbb R^d\to \mathbb R~:~ \exists w\in \ \mathbb R^d ~\text{such that}~ f(x)=x^\top w, ~\forall x \in \mathbb R^D\},
%$$
%so that finding a function $f_w$ reduces to finding a vector $w$.
Note that finding a function $f_w$ reduces to finding the corresponding vector $w$.
The term $w^\top w$ is a regularizer and helps preventing overfitting by controlling the stability of the solution. The parameter 
$\lambda$ balances the empirical error term and the regularizer. 
Equation~\eqref{eq:Tikhorls} is an instance of Tikhonov regularization,  also called 
penalized  empirical risk minimization. 
As we will see in the following, this seemingly simple example will be the basis for much more complicated solutions. 


\subsection{Computations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Consider $\ell(y, f_w(x))=(y-f_w(x))^2$.The corresponding regularized empirical risk minimization problem defines the 
%regularized least squares algorithm, a.k.a. ridge regression.
In this case, it is convenient to introduce the  input matrix $X \in \R^{n \times d}$, whose the rows are the input points, and the  output vector  $Y \in \R^{n}$ whose entries are the corresponding outputs\footnote{Note that in the 1-vs-all multiclass classification setting the output vector $Y$ becomes an $n \times T$ matrix.}. With this notation, the empirical risk can be expressed as
$$
\frac 1 n \sum_{i=1}^n (y_i-  w^\top x_i)^2=\frac 1 n \|Y- X w\|^2.
$$
A direct computation shows that the gradients with respect to $w$ of the empirical risk and the regularizer are, respectively
$$
-\frac 2 n X^\top (Y- X w), \quad \text{and} \quad 2 w.
$$
Then, setting the gradient to zero,  we have that the solution of regularized least squares solves the linear system
$$
(X^\top X+ n \lambda  I_n)w= X^\top Y,
$$
where $I_n$ is the $n \times n$ identity matrix.
Several comments are in order.
First, several methods can be used to solve the above linear system, Cholesky decomposition being the method of choice, since the matrix
 $X^\top X+\lambda I_n$ is symmetric and positive definite. 
%The \texttt{backslash} command should be used in matlab. 
The complexity of the method is essentially $O(nd^2)$ for training
and $O(d)$ for testing. The parameter $\lambda$ controls the {\em invertibility} of the matrix  
$(X^\top X+ n \lambda  I_n)$. 






%\subsection{Dealing with an Offset}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%When considering linear models, especially in relatively low dimensional spaces, it is interesting to consider an offset $b$, that is 
%$f=w^\top x+b$. We shall ask the question of how to estimate $b$ from data.
%A simple idea is to simply augment the dimension of the input space, considering  $\tilde{x}=(x,1)$ and $\tilde{w}=(w,b)$. 
%While this is  fine if we do not regularize, if we do then we still tend to prefer linear functions passing through the origin, since the regularizer becomes
%$$
%\|\tilde{w}\|^2=\|w\|^2+b^2.
%$$  
%Note that it penalizes the offset, which is not ok! In general we might not have reasons to believe that the model should pass through the origin, hence we would like to consider
%an offset  and still regularize considering only $\|w\|^2$, so that  the offset is not penalized. Note that the regularized problem becomes 
%$$
%\min_{(w,b)\in \mathbb R^{d+1}}\frac 1 n \sum_{i=1}^n (y_i- w^\top  x_i-b)^2+\lambda \|w\|^2.
%$$
%The solution of the above problem is particularly simple when considering  least squares. Indeed, in this case 
%it can be easily proved that a solution $w^*, b^*$ of the above problem is given by 
%$$
%b^*=\bar{y}-\bar{x}^\top w^*
%$$
%where $\bar y =\frac 1 n \sum_{i=1}^n y_i$, $\bar x =\frac 1 n \sum_{i=1}^n x_i$  and $w^*$ solves
%$$
%\min_{w\in \mathbb R^{d+1}}\frac 1 n \sum_{i=1}^n (y^c_i-  w^\top x^c_i)^2+\lambda \|w\|^2.
%$$
%where $y^c_i=y-\bar y$ and $x^c_i=x-\bar x$ for all $i=1, \dots, n$.

